Learning to Embed Words in Context for Syntactic Tasks

We present models for embedding words in the context of surrounding words. Such models, which we refer to as token embeddings, represent the characteristics of a word that are specific to a given context, such as word sense, syntactic category, and semantic role. We explore simple, efficient token embedding models based on standard neural network architectures. We learn token embeddings on a large amount of unannotated text and evaluate them as features for part-of-speech taggers and dependency parsers trained on much smaller amounts of annotated data. We find that predictors endowed with token embeddings consistently outperform baseline predictors across a range of context window and training set sizes.

==> losses.tex <==
\section{Training Criteria}
\label{sec:losses}

We now discuss ways of training the encoders from Sec.~\ref{sec:models}. 

We are given only a corpus $X = \{\senti \}_{i=1}^{|X|}$ of word sequences, each of which may be a sentence, paragraph, or document. 

Reconstruction error and its variants form one commonly-used family of unsupervised learning criteria for representation learning. For example, they are used when training autoencoders, which use an encoder $\enc$ to convert the input $\sent$ to a vector followed by a decoder $\dec$ that attempts to reconstruct the input from the vector.  

The typical loss function is the squared difference between the input and reconstructed input.

We use a generalization that is sensitive to the position of elements.  Since our primary interest is in learning useful representations for a \emph{particular} token in its context, 
%while $\lossre$ weights the reconstruction of all tokens equally. So 
we propose to use a weighted reconstruction error:
%\vspace{-.1in}
\begin{equation}
\textstyle
\losswre(\enc,\dec,\sent,j) = \sum_{i=1}^{|\sent|} \omega_i\left\| \dec(\encfull)_i - \vect{v}_{x_i} \right\|_2^2 \label{eq:reconst}
\end{equation}
%\vspace{-.1in}
\noindent where $\dec(\encfull)_i$ is the subvector of $\dec(\encfull)$ corresponding to reconstructing 
%the $i$th entry 
$\vect{v}_{x_i}$, and where $\omega_i$ is the weight for reconstructing the $i$th entry.


For our DNN encoder, we use analogous fully-connected layers in the decoder $\dec$. This forms a standard autoencoder architecture. For our LSTM encoder, we use the LSTM architecture for the decoder $\dec$ to reconstruct the original type embedding with weighted squared loss. 

While popular, reconstruction error 
requires a separate decoder that inverts the process of the encoder.

Other losses are possible within the framework of reconstruction-based training, such as cross-entropy/log loss.  
Squared error has the advantage that it avoids a costly summation over the vocabulary, and is still well-defined when the vocabulary is unbounded (e.g., when using subword information to define word type embeddings). 

